Real-Time Driver Monitoring Systems through Modality and View Analysis

Driver distractions are known to be the dominant cause of road accidents. While monitoring systems can detect non-driving-related activities and facilitate reducing the risks, they must be accurate and efficient to be applicable. Unfortunately, state-of-the-art methods prioritize accuracy while ignoring latency because they leverage cross-view and multimodal videos in which consecutive frames are highly similar. Thus, in this paper, we pursue time-effective detection models by neglecting the temporal relation between video frames and investigate the importance of each sensing modality in detecting drives' activities. Experiments demonstrate that 1) our proposed algorithms are real-time and can achieve similar performances (97.5\% AUC-PR) with significantly reduced computation compared with video-based models; 2) the top view with the infrared channel is more informative than any other single modality. Furthermore, we enhance the DAD dataset by manually annotating its test set to enable multiclassification. We also thoroughly analyze the influence of visual sensor types and their placements on the prediction of each class. The code and the new labels will be released.

==> 3-methods/2-loss.tex <==
\subsection{The Posterior Cross-Entropy Loss}
\label{sec:3.2}

As illustrated in Table \ref{tbl:3}, in training, there are seven categories of activities ($c_1$ -- $c_7$) to classify. The first activity, ``normal driving'' ($c_1$), means the subject is not engaging in any non-driving-related activities while the rest ($c_2$ -- $c_7$) means the opposite. During the test time, models are expected to also recognise any unseen NDRAs ($c_8$): they may not be able to tell which specific kind of activities, but they should predict that the driver is at least not driving attentively. To cover this situation, we propose a new training loss function based on conditional probability and cross entropy.

For any arbitrary model with the output $\boldsymbol{y}^{\text{pred}} \in \mathbb{R}^7$, we interpret it as
\begin{equation}
    \label{eqn:1}
    \boldsymbol{y}^{\text{pred}} =
    \begin{bmatrix}
        \mathbb{P}[c_1] & \\
        \mathbb{P}\left[c_2 \;\middle|\; \text{NDRA}\right] & \\
        \vdots & \\
        \mathbb{P}\left[c_7 \;\middle|\; \text{NDRA}\right] &
    \end{bmatrix} \in \mathbb{R}^7,
\end{equation}
where $c_i$ ($i=1, \, \cdots, \, 7$) represent the classes in the training set (as specified in Table \ref{tbl:3}), $\mathbb{P}[c_1]$ stands for the probability of the class $c_1$, and $\mathbb{P}\left[c_i \;\middle|\; \text{NDRA}\right]$ ($i = 2, \, \cdots, 7$) means the probability of the class $c_i$ given that the class is a NDRA with $\sum_{i=2}^7 \mathbb{P}\left[c_i \;\middle|\; \text{NDRA}\right] = 1$.

Notice that for $i = 2, \, \cdots, 7$,
\begin{align}
    \mathbb{P}[c_i] = & \mathbb{P}[c_i \cap \text{NDRA}] \notag \\
    = & \mathbb{P}\left[c_i \;\middle|\; \text{NDRA}\right] \cdot \mathbb{P}[\text{NDRA}] \notag \\
    = & \boldsymbol{y}^{\text{pred}}_{i} \cdot (1 - \boldsymbol{y}^{\text{pred}}_{1}) \label{eqn:2}
\end{align}

Suppose $\boldsymbol{y}^{\text{true}}$ is the one-hot encoded vector. Based on \eqref{eqn:2}, we can calculate the cross-entropy loss
\begin{align}
& l(\boldsymbol{y}^{\text{pred}}, \; \boldsymbol{y}^{\text{true}}) \notag \\
= & - \sum_{i=1}^7 \mathbbm{1}(\boldsymbol{y}^{\text{true}} = \boldsymbol{1}_i) \cdot \ln{\mathbb{P}[c_i]} \notag\\
= & - \mathbbm{1}(\boldsymbol{y}^{\text{true}} = \boldsymbol{1}_1) \cdot \ln{\boldsymbol{y}^{\text{pred}}_1} - \notag \\
& \sum_{i=2}^7 \mathbbm{1}(\boldsymbol{y}^{\text{true}} = \boldsymbol{1}_i) \cdot \ln \left( \boldsymbol{y}^{\text{pred}}_{i} \cdot (1 - \boldsymbol{y}^{\text{pred}}_{1}) \right), \label{eqn:3}
\end{align}
where $\boldsymbol{1}_i$ is the vector with the $i$-th component being 1 and the rest being 0, and $\mathbbm{1}(\cdot)$ is the indicator function.

In the test time, we can threshold $\boldsymbol{y}^{\text{pred}}$ to make prediction. Let $0 \le t_1, \, t_2 \le 1$ be two thresholds. If $\boldsymbol{y}^{\text{pred}}_1 \ge t_1$, then the predicted class is $c_1$; otherwise it is a NDRA. In the latter case, if $\max \{ \boldsymbol{y}^{\text{pred}}_{2}, \, \cdots, \, \boldsymbol{y}^{\text{pred}}_{7}\} \ge t_2$, then the predition is the corresponding class with the maximum probability; otherwise, it is an unseen NDRA ($c_8$). Notice that we can actually extend this method to the case where there are multiple classes having unseen subclasses. See Supplementary for details.

==> 4-experiments/5-visualisations.tex <==
\subsection{Visualisations of Attention Heatmaps}

==> 4-experiments/7-contrastive-learning.tex <==
\subsection{Effectiveness of Contrastive Learning}

We leverage contrastive learning \cite{khosla2020supervised} to train our base encoders and our proposed posterior cross-entropy loss to concurrently but separately train the classifier. In this section, we demonstrate that compared with solely leveraging the posterior cross-entropy loss, including the supervised contrastive loss helps our models generate better. We exploit the feature-level fusion method and employ ResNet-18 \cite{he2016deep} as the base encoder. From Table \ref{tbl:contrast}, we can reach the same conclusion from \cite{kopuklu2021driver}: despite the modality, contrastive learning can consistently ehance models' performances in this open-set recognition problem .

\input{floats/tbl_contrast}


==> floats/fig_aff.tex <==
\begin{figure}[tb]
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{images/model_structures/AFF.png}}
    \centerline{(c) AFF.}\medskip
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\linewidth}
    \centering
    \centerline{\includegraphics[width=\linewidth]{images/model_structures/iAFF.png}}
    \centerline{(d) Iterative-AFF.}\medskip
\end{minipage}
\caption{The mechansims of AFF and iAFF \cite{dai2021attentional}.}
\label{fig:aff}
\end{figure}


==> floats/fig_orig_ms_cam.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/model_structures/MSCAM.png}
    \caption{The structures of the \textit{multi-scale feature fusion module} (MC-CAM) proposed in \cite{dai2021attentional}. The feature $\boldsymbol{X}$ is passed to two different branches. One leverages the global average pooling to extract global information, while the other focuses on local details. Then these extracted features are summed together and passed to the sigmoid function to generate channel-wise weights.}
    \label{fig:orig_ms_cam}
\end{figure}


==> floats/tbl_contrast.tex <==
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc}
\hline
\multirow{2}{*}{\textbf{Modality}} & \multicolumn{2}{c}{\textbf{Method}}            \\ \cline{2-3} 
                                   & \textbf{SupConLoss + PostCE} & \textbf{PostCE} \\ \hline
Top Depth                          & \textbf{95.8}                & 94.7            \\
Top IR                             & \textbf{96.0}                & 95.2            \\
Top (Depth + IR)                   & \textbf{95.7}                & 95.0            \\ \hline
Front Depth                        & \textbf{91.9}                & 91.2            \\
Front IR                           & \textbf{91.9}                & 90.3            \\
Front (Depth + IR)                 & \textbf{93.0}                & 92.2            \\ \hline
(Top + Front) Depth                & \textbf{95.9}                & 95.4            \\
(Top + Front) IR                   & \textbf{96.7}                & 96.5            \\
(Top + Front) (Depth + IR)         & \textbf{97.1}                & 96.0            \\ \hline
\end{tabular}}
\caption{The AUC-PR values of models trained with two disparate loss functions. We can see leveraging the contrastive learning to tune the base encoder always leads to a better result.}
\label{tbl:contrast}
\end{table}

